Beyond Euclidean Summaries: Online Change Point Detection for Distribution-Valued Data

Existing online change-point detection (CPD) methods rely on fixed-dimensional Euclidean summaries, implicitly assuming that distributional changes are well captured by moment-based or feature-based representations. They can obscure important changes in distributional shape or geometry. We propose an intrinsic distribution-valued CPD framework that treats streaming batch data as a stochastic process on the 2-Wasserstein space. Our method detects changes in the law of this process by mapping each empirical distribution to a tangent space relative to a pre-change Fr\'echet barycenter, yielding a reference-centered local linearization of 2-Wasserstein space. This representation enables sequential detectors by adapting classical multivariate monitoring statistics to tangent fields. We provide theoretical guarantees and demonstrate, via synthetic and real-world experiments, that our approach detects complex distributional shifts with reduced detection delay at matched $\mathrm{ARL}_0$ compared with moments-based and model-free baselines. The code is available at https://github.com/yyzeng43/IDD-icml .

==> arixv/tables/Implementation_Details.tex <==
\begin{table*}[t]
\centering
\caption{\rev{Example implementation details and hyperparameters used across our experiments. CNF stands for Conditional Normalizing Flows.}}
\label{tab:implementation_details}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccccc}
\toprule
 & Synthetic ($d{=}1$) & Synthetic ($d{=}5$) & Synthetic ($d{=}10$) & Synthetic ($d{=}50$) & FlowCAP-II (AML) & Reddit Sentiment \\
\midrule
\multicolumn{7}{l}{\textbf{Data}} \\
Dimension $d$        & 1 & 5 & 10 & 50 & 7 & 20 \\
Batch size $N_t$     & \{50, 100, 300\} & \{50, 100, 300\} & \{50, 100, 300\} & \{50, 100, 300\} & $\sim$100--300 & $\sim$50--200 \\
Pre-change $n_0$     & 300 & 300 & 300 & 300 & 300 & 50 \\
MFPCA trunc.\ $K$    & CVE $\ge 0.95$ & CVE $\ge 0.95$ & CVE $\ge 0.95$ & CVE $\ge 0.95$ & CVE $\ge 0.95$ & CVE $\ge 0.95$ \\
\midrule
\multicolumn{7}{l}{\textbf{OT Solver}} \\
Method               & Exact LP & Exact LP & Sinkhorn & Sinkhorn & Sinkhorn & Sinkhorn \\
Library call         & \texttt{ot.emd()} & \texttt{ot.emd()} & \texttt{ot.sinkhorn()} & \texttt{ot.sinkhorn()} & \texttt{ot.sinkhorn()} & \texttt{ot.sinkhorn()} \\
\texttt{reg} ($\varepsilon$) & --- & --- & 0.05 & 0.05 & 0.05 & 0.05 \\
\texttt{numIterMax}  & --- & --- & 5000 & 5000 & 5000 & 5000 \\
\texttt{stopThr}     & --- & --- & 1e-4 & 1e-4 & 1e-4 & 1e-4 \\
\texttt{use\_eps\_scaling} & --- & --- & True & True & True & True \\
\midrule
\multicolumn{7}{l}{\textbf{Barycenter}} \\
Method               & Closed-form & Fixed-support Sinkhorn & CNF & CNF & CNF & CNF \\
\texttt{n\_bary}     & --- & 512 & --- & --- & --- & --- \\
Sinkhorn inner iters & --- & 500 & --- & --- & --- & --- \\
Fixed-point outer iters & --- & 300 & --- & --- & --- & --- \\
\texttt{flow\_bar\_hidden}   & --- & --- & 32 & 32 & 32 & 32 \\
\texttt{flow\_bar\_blocks}   & --- & --- & 8  & 8  & 8  & 8  \\
\texttt{flow\_ot\_hidden}    & --- & --- & 64 & 64 & 64 & 64 \\
\texttt{flow\_ot\_blocks}    & --- & --- & 16 & 16 & 16 & 16 \\
\texttt{epochs}      & --- & --- & 500  & 500  & 500  & 500  \\
\texttt{batch\_size} (train) & --- & --- & 2048 & 2048 & 2048 & 2048 \\
\texttt{lr}          & --- & --- & 1e-3 & 1e-3 & 1e-3 & 1e-3 \\
\texttt{grad\_clip}  & --- & --- & 2.0  & 2.0  & 2.0  & 2.0  \\
Temp.\ schedule      & --- & --- & $1.0 \to 10^{-2}$ & $1.0 \to 10^{-2}$ & $1.0 \to 10^{-2}$ & $1.0 \to 10^{-2}$ \\
LR scheduler         & --- & --- & Plateau (0.8, pat=1000) & Plateau (0.8, pat=1000) & Plateau (0.8, pat=1000) & Plateau (0.8, pat=1000) \\
\bottomrule
\end{tabular}}
\end{table*}


==> arixv/tables/KDE_marginal.tex <==
\begin{table}[t]
\centering
\caption{\rev{Synthetic results for the \textbf{Copula Shift} scenario comparing the proposed OT-based detector against a KDE-Marginal baseline that monitors per-coordinate marginal densities via functional $L^2$ distances. For each $(N,d,K)$ configuration, the row with the smaller mean $\mathrm{ARL}_1$ is highlighted in bold.}}
\label{tab:kde_marginal}
\resizebox{0.5\linewidth}{!}{%
\begin{tabular}{lccccc}
\toprule
Method & $N$ & $d$ & $K$ & $\mathrm{ARL}_1$ (mean) & $\mathrm{ARL}_1$ (SE) \\
\midrule
KDE-Marginal & 50 & 1 & 4 & 16.600 & 2.729 \\
\rowcolor{gray!12}
\textbf{OT (Ours)} & \textbf{50} & \textbf{1} & \textbf{4} & \textbf{10.800} & \textbf{3.782} \\
KDE-Marginal & 50 & 5 & 4 & 13.700 & 3.073 \\
\rowcolor{gray!12}
\textbf{OT (Ours)} & \textbf{50} & \textbf{5} & \textbf{4} & \textbf{1.100} & \textbf{0.100} \\
KDE-Marginal & 50 & 10 & 4 & 6.600 & 1.507 \\
\rowcolor{gray!12}
\textbf{OT (Ours)} & \textbf{50} & \textbf{10} & \textbf{4} & \textbf{1.000} & \textbf{0.000} \\
KDE-Marginal & 50 & 50 & 4 & 8.400 & 1.454 \\
\rowcolor{gray!12}
\textbf{OT (Ours)} & \textbf{50} & \textbf{50} & \textbf{4} & \textbf{1.000} & \textbf{0.000} \\
\midrule
KDE-Marginal & 100 & 1 & 4 & 13.100 & 2.927 \\
\rowcolor{gray!12}
\textbf{OT (Ours)} & \textbf{100} & \textbf{1} & \textbf{4} & \textbf{10.800} & \textbf{4.482} \\
KDE-Marginal & 100 & 5 & 4 & 8.700 & 1.535 \\
\rowcolor{gray!12}
\textbf{OT (Ours)} & \textbf{100} & \textbf{5} & \textbf{4} & \textbf{1.000} & \textbf{0.000} \\
KDE-Marginal & 100 & 10 & 4 & 16.000 & 4.222 \\
\rowcolor{gray!12}
\textbf{OT (Ours)} & \textbf{100} & \textbf{10} & \textbf{4} & \textbf{1.000} & \textbf{0.000} \\
KDE-Marginal & 100 & 50 & 4 & 17.800 & 3.759 \\
\rowcolor{gray!12}
\textbf{OT (Ours)} & \textbf{100} & \textbf{50} & \textbf{4} & \textbf{1.000} & \textbf{0.000} \\
\midrule
KDE-Marginal & 300 & 1 & 4 & 13.900 & 3.816 \\
\rowcolor{gray!12}
\textbf{OT (Ours)} & \textbf{300} & \textbf{1} & \textbf{4} & \textbf{9.500} & \textbf{3.622} \\
KDE-Marginal & 300 & 5 & 4 & 11.300 & 2.305 \\
\rowcolor{gray!12}
\textbf{OT (Ours)} & \textbf{300} & \textbf{5} & \textbf{4} & \textbf{1.000} & \textbf{0.000} \\
KDE-Marginal & 300 & 10 & 4 & 7.800 & 1.775 \\
\rowcolor{gray!12}
\textbf{OT (Ours)} & \textbf{300} & \textbf{10} & \textbf{4} & \textbf{1.000} & \textbf{0.000} \\
KDE-Marginal & 300 & 50 & 4 & 9.600 & 1.933 \\
\rowcolor{gray!12}
\textbf{OT (Ours)} & \textbf{300} & \textbf{50} & \textbf{4} & \textbf{1.000} & \textbf{0.000} \\
\bottomrule
\end{tabular}}
\end{table}


==> arixv/tables/PhaseII_timing.tex <==
\begin{table}[t]
\centering
\caption{\rev{Phase II online deployment time for synthetic continuous-stream experiments. Units are ms per sample; entries are mean (SE). Phase II values are averaged over MM reweight, Copula shift, and Barycenter scenarios.}}
\label{tab:phaseII_timing}
\resizebox{\linewidth}{!}{%
\begin{tabular}{cccccccccc}
\toprule
$N$ & $d$ & $K$ & OT & KDE-Full & KDE-Marginal & $\bar X$/Hotelling $T^2$ & NEWMA & Scan-B & F-CPD \\
\midrule
50  & 1  & 4 & 0.212 (0.006)   & 0.969 (0.016) & 0.958 (0.013)   & 0.009 (0.000) & 0.206 (0.002) & 0.436 (0.002) & 12.246 (0.559) \\
50  & 5  & 4 & 17.313 (0.332)  & 0.947 (0.006) & 4.436 (0.018)   & 0.023 (0.000) & 0.228 (0.001) & 0.461 (0.004) & 11.667 (0.022) \\
50  & 10 & 4 & 26.433 (0.872)  & 0.998 (0.004) & 8.680 (0.015)   & 0.042 (0.000) & 0.249 (0.001) & 0.484 (0.001) & 12.027 (0.115) \\
50  & 50 & 4 & 31.265 (0.995)  & 1.599 (0.007) & 48.446 (0.041)  & 0.227 (0.002) & 1.452 (0.094) & 1.672 (0.086) & 12.884 (0.092) \\
\midrule
100 & 1  & 4 & 0.243 (0.021)   & 1.358 (0.013) & 1.375 (0.009)   & 0.013 (0.000) & 0.379 (0.003) & 0.619 (0.003) & 13.733 (0.022) \\
100 & 5  & 4 & 29.651 (0.717)  & 1.709 (0.010) & 6.964 (0.020)   & 0.046 (0.001) & 0.444 (0.002) & 0.687 (0.006) & 13.994 (0.033) \\
100 & 10 & 4 & 47.805 (1.633)  & 1.885 (0.008) & 13.503 (0.063)  & 0.096 (0.002) & 0.495 (0.003) & 0.725 (0.003) & 13.407 (0.025) \\
100 & 50 & 4 & 48.868 (1.763)  & 3.409 (0.009) & 72.002 (0.080)  & 0.484 (0.009) & 2.839 (0.015) & 2.983 (0.069) & 16.183 (0.115) \\
\midrule
300 & 1  & 4 & 0.272 (0.003)   & 3.295 (0.024) & 3.440 (0.043)   & 0.030 (0.001) & 1.120 (0.007) & 1.387 (0.011) & 15.498 (0.101) \\
300 & 5  & 4 & 170.580 (6.157) & 4.511 (0.030) & 17.983 (0.169)  & 0.154 (0.003) & 3.919 (0.023) & 4.141 (0.018) & 18.152 (0.136) \\
300 & 10 & 4 & 236.114 (8.591) & 4.993 (0.020) & 35.330 (0.212)  & 0.294 (0.003) & 2.994 (0.058) & 3.780 (0.037) & 17.118 (0.114) \\
300 & 50 & 4 & 272.048 (11.912)& 8.863 (0.052) & 171.644 (0.981) & 1.409 (0.006) & 4.548 (0.071) & 5.100 (0.030) & 20.158 (0.115) \\
\bottomrule
\end{tabular}}
\end{table}


==> arixv/tables/PhaseI_timing.tex <==
\begin{table}[t]
\centering
\caption{\rev{Phase I calibration time for synthetic continuous-stream experiments. Units are ms per sample; entries are mean (SE).}}
\label{tab:phaseI_timing}
\resizebox{\linewidth}{!}{%
\begin{tabular}{cccccccccc}
\toprule
$N$ & $d$ & $K$ & OT & KDE-Full & KDE-Marginal & $\bar X$/Hotelling $T^2$ & NEWMA & Scan-B & F-CPD \\
\midrule
50  & 1  & 4 & 0.184 (0.007)   & 0.911 (0.012) & 0.919 (0.017)   & 0.010 (0.000) & 0.205 (0.002) & 0.400 (0.003) & 6.864 (0.045)  \\
50  & 5  & 4 & 292.124 (4.869) & 0.903 (0.008) & 4.354 (0.045)   & 0.023 (0.000) & 0.230 (0.001) & 0.411 (0.003) & 6.816 (0.020)  \\
50  & 10 & 4 & 332.594 (0.575) & 0.983 (0.009) & 8.496 (0.017)   & 0.041 (0.000) & 0.253 (0.001) & 0.439 (0.004) & 6.989 (0.071)  \\
50  & 50 & 4 & 480.422 (0.799) & 1.591 (0.015) & 42.363 (0.059)  & 0.234 (0.000) & 1.197 (0.099) & 1.537 (0.113) & 8.112 (0.077)  \\
\midrule
100 & 1  & 4 & 0.204 (0.006)   & 1.341 (0.006) & 1.343 (0.005)   & 0.014 (0.000) & 0.383 (0.002) & 0.588 (0.009) & 7.894 (0.024)  \\
100 & 5  & 4 & 303.171 (0.507) & 1.680 (0.008) & 6.813 (0.011)   & 0.044 (0.000) & 0.451 (0.002) & 0.642 (0.004) & 8.150 (0.021)  \\
100 & 10 & 4 & 377.411 (0.923) & 1.856 (0.005) & 13.465 (0.032)  & 0.095 (0.000) & 0.489 (0.003) & 0.686 (0.004) & 7.765 (0.024)  \\
100 & 50 & 4 & 501.894 (0.892) & 3.374 (0.010) & 67.953 (0.166)  & 0.482 (0.000) & 2.790 (0.021) & 2.969 (0.045) & 10.440 (0.088) \\
\midrule
300 & 1  & 4 & 0.316 (0.026)   & 3.355 (0.010) & 3.549 (0.100)   & 0.031 (0.000) & 1.135 (0.008) & 1.333 (0.009) & 9.496 (0.060)  \\
300 & 5  & 4 & 477.198 (4.262) & 4.465 (0.026) & 17.803 (0.138)  & 0.149 (0.000) & 3.898 (0.033) & 4.141 (0.061) & 11.889 (0.065) \\
300 & 10 & 4 & 727.812 (8.781) & 4.966 (0.014) & 37.531 (1.378)  & 0.294 (0.000) & 3.038 (0.055) & 3.742 (0.050) & 11.412 (0.114) \\
300 & 50 & 4 & 866.880 (21.230)& 8.891 (0.037) & 175.223 (1.749) & 1.410 (0.000) & 4.914 (0.041) & 4.935 (0.077) & 13.517 (0.308) \\
\bottomrule
\end{tabular}}
\end{table}


==> arixv/tables/Syn_con1.tex <==
\begin{table}[htbp]
    \centering
    % --- Left: Barycenter d=1 ---
    \begin{minipage}[htbp]{0.48\linewidth}
        \centering
        \caption{Synthetic results for \textbf{Barycenter} with $d=1$ (10 replications). Best (smallest) \arlo is bold.}
        \label{tab:syn:barycenter:d1}
        \resizebox{0.9\linewidth}{!}{%
        \begin{tabular}{lcccc}
            \toprule
            Method & $N$ & \arlz (emp) & \arlo \\
            \midrule
            F-CPD & 50 & 79.8 & 3.3 $\pm$ 0.7 \\
            Log-KDE & 50 & 99.4 & 1.1 $\pm$ 0.1 \\
            NEWMA & 50 & 101.6 & 2.4 $\pm$ 0.4 \\
            \rowcolor{gray!12}
            Ours & 50 & 102.9 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$9.1\%)}} \\
            Scan-B & 50 & 101.1 & 3.4 $\pm$ 0.4 \\
            Shewhart & 50 & 99.2 & 232.1 $\pm$ 39.5 \\
            \midrule
            F-CPD & 100 & 81.5 & 3.2 $\pm$ 0.3 \\
            Log-KDE & 100 & 104.4 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$47.4\%)}} \\
            NEWMA & 100 & 111.9 & 1.9 $\pm$ 0.4 \\
            \rowcolor{gray!12}
            Ours & 100 & 103.4 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$47.4\%)}} \\
            Scan-B & 100 & 101.2 & 2.9 $\pm$ 0.4 \\
            Shewhart & 100 & 103.7 & 241.0 $\pm$ 40.0 \\
            \midrule
            F-CPD & 300 & 94.2 & 3.0 $\pm$ 0.0 \\
            Log-KDE & 300 & 101.6 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$23.1\%)}} \\
            NEWMA & 300 & 105.5 & 1.3 $\pm$ 0.2 \\
            \rowcolor{gray!12}
            Ours & 300 & 107.2 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$23.1\%)}} \\
            Scan-B & 300 & 97.1 & 2.1 $\pm$ 0.2 \\
            Shewhart & 300 & 97.0 & 241.0 $\pm$ 40.0 \\
            \bottomrule
        \end{tabular}}
    \end{minipage}
    \hfill
    % --- Right: Barycenter d=5 ---
    \begin{minipage}[htbp]{0.48\linewidth}
        \centering
        \caption{Synthetic results for \textbf{Barycenter} with $d=5$ (10 replications). Best (smallest) \arlo is bold.}
        \label{tab:syn:barycenter:d5}
        \resizebox{0.9\linewidth}{!}{%
        \begin{tabular}{lcccc}
            \toprule
            Method & $N$ & \arlz (emp) & \arlo \\
            \midrule
            F-CPD & 50 & 93.6 & 2.8 $\pm$ 0.2 \\
            Log-KDE & 50 & 107.2 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$28.6\%)}} \\
            NEWMA & 50 & 90.8 & 1.4 $\pm$ 0.2 \\
            \rowcolor{gray!12}
            Ours & 50 & 101.6 & 1.8 $\pm$ 0.5 \\
            Scan-B & 50 & 98.7 & 2.2 $\pm$ 0.1 \\
            Shewhart & 50 & 105.3 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$28.6\%)}} \\
            \midrule
            F-CPD & 100 & 102.1 & 3.0 $\pm$ 0.0 \\
            Log-KDE & 100 & 97.8 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$52.4\%)}} \\
            NEWMA & 100 & 98.8 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$52.4\%)}} \\
            \rowcolor{gray!12}
            Ours & 100 & 99.7 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$52.4\%)}} \\
            Scan-B & 100 & 96.0 & 2.1 $\pm$ 0.1 \\
            Shewhart & 100 & 104.4 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$52.4\%)}} \\
            \midrule
            F-CPD & 300 & 100.4 & 2.6 $\pm$ 0.3 \\
            Log-KDE & 300 & 100.6 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$41.2\%)}} \\
            NEWMA & 300 & 100.7 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$41.2\%)}} \\
            \rowcolor{gray!12}
            Ours & 300 & 95.5 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$41.2\%)}} \\
            Scan-B & 300 & 95.0 & 1.7 $\pm$ 0.2 \\
            Shewhart & 300 & 101.6 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$41.2\%)}} \\
            \bottomrule
        \end{tabular}}
    \end{minipage}
\end{table}

==> arixv/tables/Syn_con2.tex <==
\begin{table}[htbp]
    \centering
    % --- Left: Barycenter d=10 ---
    \begin{minipage}[htbp]{0.48\linewidth}
        \centering
        \caption{Synthetic results for \textbf{Barycenter} with $d=10$ (10 replications). Best (smallest) \arlo is bold.}
        \label{tab:syn:barycenter:d10}
        \resizebox{0.9\linewidth}{!}{%
        \begin{tabular}{lcccc}
            \toprule
            Method & $N$ & \arlz (emp) & \arlo \\
            \midrule
            F-CPD & 50 & 94.3 & 3.0 $\pm$ 0.0 \\
            Log-KDE & 50 & 104.3 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$16.7\%)}} \\
            NEWMA & 50 & 100.8 & 1.2 $\pm$ 0.1 \\
            \rowcolor{gray!12}
            Ours & 50 & 101.2 & 3.0 $\pm$ 1.9 \\
            Scan-B & 50 & 93.3 & 2.0 $\pm$ 0.0 \\
            Shewhart & 50 & 92.9 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$16.7\%)}} \\
            \midrule
            F-CPD & 100 & 99.0 & 3.0 $\pm$ 0.0 \\
            Log-KDE & 100 & 108.2 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$50.0\%)}} \\
            NEWMA & 100 & 101.1 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$50.0\%)}} \\
            \rowcolor{gray!12}
            Ours & 100 & 95.9 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$50.0\%)}} \\
            Scan-B & 100 & 100.5 & 2.0 $\pm$ 0.0 \\
            Shewhart & 100 & 98.5 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$50.0\%)}} \\
            \midrule
            F-CPD & 300 & 100.1 & 3.0 $\pm$ 0.0 \\
            Log-KDE & 300 & 105.3 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$37.5\%)}} \\
            NEWMA & 300 & 100.2 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$37.5\%)}} \\
            \rowcolor{gray!12}
            Ours & 300 & 100.9 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$37.5\%)}} \\
            Scan-B & 300 & 99.8 & 1.6 $\pm$ 0.2 \\
            Shewhart & 300 & 101.0 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$37.5\%)}} \\
            \bottomrule
        \end{tabular}}
    \end{minipage}
    \hfill
    % --- Right: Barycenter d=50 ---
    \begin{minipage}[htbp]{0.48\linewidth}
        \centering
        \caption{Synthetic results for \textbf{Barycenter} with $d=50$ (10 replications). Best (smallest) \arlo is bold.}
        \label{tab:syn:barycenter:d50}
        \resizebox{0.9\linewidth}{!}{%
        \begin{tabular}{lcccc}
            \toprule
            Method & $N$ & \arlz (emp) & \arlo \\
            \midrule
            F-CPD & 50 & 101.4 & 2.6 $\pm$ 0.3 \\
            Log-KDE & 50 & 102.6 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$50.0\%)}} \\
            NEWMA & 50 & 104.0 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$50.0\%)}} \\
            \rowcolor{gray!12}
            Ours & 50 & 97.7 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$50.0\%)}} \\
            Scan-B & 50 & 101.3 & 2.0 $\pm$ 0.0 \\
            Shewhart & 50 & 95.1 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$50.0\%)}} \\
            \midrule
            F-CPD & 100 & 101.2 & 2.8 $\pm$ 0.2 \\
            Log-KDE & 100 & 94.0 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$47.4\%)}} \\
            NEWMA & 100 & 95.1 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$47.4\%)}} \\
            \rowcolor{gray!12}
            Ours & 100 & 96.8 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$47.4\%)}} \\
            Scan-B & 100 & 107.2 & 1.9 $\pm$ 0.1 \\
            Shewhart & 100 & 93.9 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$47.4\%)}} \\
            \midrule
            F-CPD & 300 & 95.1 & 3.3 $\pm$ 0.3 \\
            Log-KDE & 300 & 97.5 & 6.8 $\pm$ 2.9 \\
            NEWMA & 300 & 90.6 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$50.0\%)}} \\
            \rowcolor{gray!12}
            Ours & 300 & 110.0 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$50.0\%)}} \\
            Scan-B & 300 & 104.0 & 2.0 $\pm$ 0.0 \\
            Shewhart & 300 & 107.0 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$50.0\%)}} \\
            \bottomrule
        \end{tabular}}
    \end{minipage}
\end{table}

==> arixv/tables/Syn_con3.tex <==
\begin{table}[htbp]
    \centering
    % --- Left: Copula d=5 ---
    \begin{minipage}[htbp]{0.48\linewidth}
        \centering
        \caption{Synthetic results for \textbf{Copula Shift} with $d=5$ (10 replications). Best (smallest) \arlo is bold.}
        \label{tab:syn:copula_shift:d5}
        \resizebox{0.9\linewidth}{!}{%
        \begin{tabular}{lcccc}
            \toprule
            Method & $N$ & \arlz (emp) & \arlo \\
            \midrule
            F-CPD & 50 & 96.8 & 6.6 $\pm$ 0.7 \\
            Log-KDE & 50 & 103.2 & 2.3 $\pm$ 0.6 \\
            NEWMA & 50 & 89.3 & 3.4 $\pm$ 0.2 \\
            \rowcolor{gray!12}
            Ours & 50 & 100.1 & \textbf{1.1 $\pm$ 0.1 {\scriptsize($\uparrow$52.2\%)}} \\
            Scan-B & 50 & 98.3 & 4.3 $\pm$ 0.2 \\
            Shewhart & 50 & 99.0 & 43.1 $\pm$ 17.9 \\
            \midrule
            F-CPD & 100 & 102.0 & 4.4 $\pm$ 0.2 \\
            Log-KDE & 100 & 99.3 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$64.3\%)}} \\
            NEWMA & 100 & 91.6 & 2.8 $\pm$ 0.2 \\
            \rowcolor{gray!12}
            Ours & 100 & 91.8 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$64.3\%)}} \\
            Scan-B & 100 & 95.6 & 3.9 $\pm$ 0.2 \\
            Shewhart & 100 & 99.6 & 12.7 $\pm$ 4.2 \\
            \midrule
            F-CPD & 300 & 99.9 & 3.2 $\pm$ 0.1 \\
            Log-KDE & 300 & 116.7 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$37.5\%)}} \\
            NEWMA & 300 & 87.6 & 1.6 $\pm$ 0.2 \\
            \rowcolor{gray!12}
            Ours & 300 & 91.6 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$37.5\%)}} \\
            Scan-B & 300 & 106.6 & 2.3 $\pm$ 0.2 \\
            Shewhart & 300 & 96.3 & 35.6 $\pm$ 10.2 \\
            \bottomrule
        \end{tabular}}
    \end{minipage}
    \hfill
    % --- Right: Copula d=10 ---
    \begin{minipage}[htbp]{0.48\linewidth}
        \centering
        \caption{Synthetic results for \textbf{Copula Shift} with $d=10$ (10 replications). Best (smallest) \arlo is bold.}
        \label{tab:syn:copula_shift:d10}
        \resizebox{0.9\linewidth}{!}{%
        \begin{tabular}{lcccc}
            \toprule
            Method & $N$ & \arlz (emp) & \arlo \\
            \midrule
            F-CPD & 50 & 102.6 & 3.7 $\pm$ 0.3 \\
            Log-KDE & 50 & 96.8 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$52.4\%)}} \\
            NEWMA & 50 & 112.5 & 2.1 $\pm$ 0.1 \\
            \rowcolor{gray!12}
            Ours & 50 & 100.7 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$52.4\%)}} \\
            Scan-B & 50 & 99.9 & 3.4 $\pm$ 0.2 \\
            Shewhart & 50 & 105.7 & 2.2 $\pm$ 0.5 \\
            \midrule
            F-CPD & 100 & 108.1 & 3.8 $\pm$ 0.1 \\
            Log-KDE & 100 & 102.1 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$47.4\%)}} \\
            NEWMA & 100 & 99.6 & 1.9 $\pm$ 0.1 \\
            \rowcolor{gray!12}
            Ours & 100 & 100.2 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$47.4\%)}} \\
            Scan-B & 100 & 113.1 & 2.8 $\pm$ 0.1 \\
            Shewhart & 100 & 87.9 & 2.5 $\pm$ 0.4 \\
            \midrule
            F-CPD & 300 & 94.1 & 2.6 $\pm$ 0.3 \\
            Log-KDE & 300 & 102.2 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$44.4\%)}} \\
            NEWMA & 300 & 100.7 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$44.4\%)}} \\
            \rowcolor{gray!12}
            Ours & 300 & 91.7 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$44.4\%)}} \\
            Scan-B & 300 & 100.1 & 2.0 $\pm$ 0.0 \\
            Shewhart & 300 & 107.7 & 1.8 $\pm$ 0.3 \\
            \bottomrule
        \end{tabular}}
    \end{minipage}
\end{table}

==> arixv/tables/Syn_con4.tex <==
\begin{table}[htbp]
    \centering
    % --- Left: Copula d=50 (regenerated for camera-ready) ---
    \begin{minipage}[htbp]{0.48\linewidth}
        \centering
        \caption{\rev{Synthetic results for \textbf{Copula Shift} with $d=50$ (10 replications), regenerated for camera-ready. Best (smallest) \arlo is bold.}}
        \label{tab:syn:copula_shift:d50}
        \resizebox{0.9\linewidth}{!}{%
        \begin{tabular}{lcccc}
            \toprule
            Method & $N$ & \arlz (emp) & \arlo \\
            \midrule
            F-CPD & 50 & 100.0 & 3.1 $\pm$ 0.4 \\
            Log-KDE & 50 & 100.0 & 3.2 $\pm$ 0.7 \\
            NEWMA & 50 & 100.0 & 1.9 $\pm$ 0.1 \\
            \rowcolor{gray!12}
            Ours & 50 & 100.0 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$16.7\%)}} \\
            Scan-B & 50 & 100.0 & 2.9 $\pm$ 0.1 \\
            Shewhart & 50 & 100.0 & 1.2 $\pm$ 0.1 \\
            \midrule
            F-CPD & 100 & 100.0 & 3.4 $\pm$ 0.2 \\
            Log-KDE & 100 & 100.0 & 1.1 $\pm$ 0.1 \\
            NEWMA & 100 & 100.0 & 1.9 $\pm$ 0.1 \\
            \rowcolor{gray!12}
            Ours & 100 & 100.0 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$9.1\%)}} \\
            Scan-B & 100 & 100.0 & 2.6 $\pm$ 0.2 \\
            Shewhart & 100 & 100.0 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$9.1\%)}} \\
            \midrule
            F-CPD & 300 & 100.0 & 3.0 $\pm$ 0.0 \\
            Log-KDE & 300 & 100.0 & 4.4 $\pm$ 1.5 \\
            NEWMA & 300 & 100.0 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$50.0\%)}} \\
            \rowcolor{gray!12}
            Ours & 300 & 100.0 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$50.0\%)}} \\
            Scan-B & 300 & 100.0 & 2.0 $\pm$ 0.0 \\
            Shewhart & 300 & 100.0 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$50.0\%)}} \\
            \bottomrule
        \end{tabular}}
    \end{minipage}
    \hfill
    % --- Right: MM Reweight d=1 ---
    \begin{minipage}[htbp]{0.48\linewidth}
        \centering
        \caption{Synthetic results for \textbf{Multimodal Reweight} with $d=1$ (10 replications). Best (smallest) \arlo is bold.}
        \label{tab:syn:mm_reweight:d1}
        \resizebox{0.9\linewidth}{!}{%
        \begin{tabular}{lcccc}
            \toprule
            Method & $N$ & \arlz (emp) & \arlo \\
            \midrule
            F-CPD & 50 & 103.0 & 49.6 $\pm$ 21.6 \\
            Log-KDE & 50 & 108.3 & 45.6 $\pm$ 15.6 \\
            NEWMA & 50 & 107.9 & 24.1 $\pm$ 5.4 \\
            \rowcolor{gray!12}
            Ours & 50 & 107.7 & \textbf{15.7 $\pm$ 9.4 {\scriptsize($\uparrow$34.9\%)}} \\
            Scan-B & 50 & 93.2 & 69.7 $\pm$ 21.0 \\
            Shewhart & 50 & 101.1 & 93.5 $\pm$ 28.1 \\
            \midrule
            F-CPD & 100 & 99.5 & 59.7 $\pm$ 24.6 \\
            Log-KDE & 100 & 94.3 & \textbf{4.8 $\pm$ 1.7 {\scriptsize($\uparrow$36.8\%)}} \\
            NEWMA & 100 & 90.1 & 12.2 $\pm$ 4.1 \\
            \rowcolor{gray!12}
            Ours & 100 & 92.3 & 7.6 $\pm$ 4.0 \\
            Scan-B & 100 & 106.2 & 70.0 $\pm$ 31.2 \\
            Shewhart & 100 & 99.9 & 36.0 $\pm$ 8.7 \\
            \midrule
            F-CPD & 300 & 99.4 & 11.8 $\pm$ 2.4 \\
            Log-KDE & 300 & 88.1 & 1.8 $\pm$ 0.5 \\
            NEWMA & 300 & 105.8 & 10.6 $\pm$ 2.6 \\
            \rowcolor{gray!12}
            Ours & 300 & 94.9 & \textbf{1.2 $\pm$ 0.2 {\scriptsize($\uparrow$33.3\%)}} \\
            Scan-B & 300 & 109.5 & 11.1 $\pm$ 4.2 \\
            Shewhart & 300 & 94.5 & 108.0 $\pm$ 20.6 \\
            \bottomrule
        \end{tabular}}
    \end{minipage}
\end{table}

==> arixv/tables/Syn_con5.tex <==
\begin{table}[htbp]
    \centering
    % --- Left: MM Reweight d=5 ---
    \begin{minipage}[htbp]{0.48\linewidth}
        \centering
        \caption{Synthetic results for \textbf{Multimodal Reweight} with $d=5$ (10 replications). Best (smallest) \arlo is bold.}
        \label{tab:syn:mm_reweight:d5}
        \resizebox{0.9\linewidth}{!}{%
        \begin{tabular}{lcccc}
            \toprule
            Method & $N$ & \arlz (emp) & \arlo \\
            \midrule
            F-CPD & 50 & 96.8 & 66.2 $\pm$ 29.4 \\
            Log-KDE & 50 & 103.2 & 85.4 $\pm$ 34.4 \\
            NEWMA & 50 & 89.3 & 28.2 $\pm$ 6.1 \\
            \rowcolor{gray!12}
            Ours & 50 & 100.1 & \textbf{25.5 $\pm$ 9.5 {\scriptsize($\uparrow$6.9\%)}} \\
            Scan-B & 50 & 98.3 & 27.4 $\pm$ 8.6 \\
            Shewhart & 50 & 99.0 & 145.3 $\pm$ 36.6 \\
            \midrule
            F-CPD & 100 & 102.0 & 21.1 $\pm$ 4.3 \\
            Log-KDE & 100 & 99.3 & 40.1 $\pm$ 14.7 \\
            NEWMA & 100 & 91.6 & 18.6 $\pm$ 6.8 \\
            \rowcolor{gray!12}
            Ours & 100 & 91.8 & \textbf{10.0 $\pm$ 4.4 {\scriptsize($\uparrow$46.2\%)}} \\
            Scan-B & 100 & 95.6 & 72.3 $\pm$ 32.6 \\
            Shewhart & 100 & 99.6 & 92.9 $\pm$ 26.6 \\
            \midrule
            F-CPD & 300 & 99.9 & 9.7 $\pm$ 1.0 \\
            Log-KDE & 300 & 116.7 & 6.3 $\pm$ 4.5 \\
            NEWMA & 300 & 87.6 & 6.5 $\pm$ 0.8 \\
            \rowcolor{gray!12}
            Ours & 300 & 91.6 & \textbf{3.1 $\pm$ 1.1 {\scriptsize($\uparrow$50.8\%)}} \\
            Scan-B & 300 & 106.6 & 6.8 $\pm$ 0.6 \\
            Shewhart & 300 & 96.3 & 190.8 $\pm$ 40.5 \\
            \bottomrule
        \end{tabular}}
    \end{minipage}
    \hfill
    % --- Right: MM Reweight d=10 ---
    \begin{minipage}[htbp]{0.48\linewidth}
        \centering
        \caption{Synthetic results for \textbf{Multimodal Reweight} with $d=10$ (10 replications). Best (smallest) \arlo is bold.}
        \label{tab:syn:mm_reweight:d10}
        \resizebox{0.9\linewidth}{!}{%
        \begin{tabular}{lcccc}
            \toprule
            Method & $N$ & \arlz (emp) & \arlo \\
            \midrule
            F-CPD & 50 & 102.6 & 17.7 $\pm$ 5.2 \\
            Log-KDE & 50 & 96.8 & 16.4 $\pm$ 10.2 \\
            NEWMA & 50 & 112.5 & 11.3 $\pm$ 3.4 \\
            \rowcolor{gray!12}
            Ours & 50 & 100.7 & \textbf{4.3 $\pm$ 1.9 {\scriptsize($\uparrow$61.9\%)}} \\
            Scan-B & 50 & 99.9 & 34.3 $\pm$ 17.9 \\
            Shewhart & 50 & 105.7 & 87.3 $\pm$ 25.2 \\
            \midrule
            F-CPD & 100 & 108.1 & 35.4 $\pm$ 22.2 \\
            Log-KDE & 100 & 102.1 & 29.3 $\pm$ 18.2 \\
            NEWMA & 100 & 99.6 & 10.6 $\pm$ 2.7 \\
            \rowcolor{gray!12}
            Ours & 100 & 100.2 & \textbf{1.5 $\pm$ 0.4 {\scriptsize($\uparrow$85.8\%)}} \\
            Scan-B & 100 & 113.1 & 13.0 $\pm$ 3.6 \\
            Shewhart & 100 & 87.9 & 56.0 $\pm$ 9.2 \\
            \midrule
            F-CPD & 300 & 94.1 & 4.8 $\pm$ 1.0 \\
            Log-KDE & 300 & 102.2 & 44.5 $\pm$ 30.7 \\
            NEWMA & 300 & 100.7 & 3.7 $\pm$ 0.8 \\
            \rowcolor{gray!12}
            Ours & 300 & 91.7 & \textbf{1.0 $\pm$ 0.0 {\scriptsize($\uparrow$73.0\%)}} \\
            Scan-B & 300 & 100.1 & 4.4 $\pm$ 0.7 \\
            Shewhart & 300 & 107.7 & 145.8 $\pm$ 35.1 \\
            \bottomrule
        \end{tabular}}
    \end{minipage}
\end{table}
